Convergence of score-based generative modeling for general data distributions

Score-based generative modeling (SGM) has grown to be a hugely successful method for learning to generate samples from complex data distributions such as that of images and audio. It is based on evolving an SDE that transforms white noise into a sample from the learned distribution, using estimates of the score function, or gradient log-pdf. Previous convergence analyses for these methods have suffered either from strong assumptions on the data distribution or exponential dependencies, and hence fail to give efficient guarantees for the multimodal and non-smooth distributions that arise in practice and for which good empirical performance is observed. We consider a popular kind of SGM -- denoising diffusion models -- and give polynomial convergence guarantees for general data distributions, with no assumptions related to functional inequalities or smoothness. Assuming $L^2$-accurate score estimates, we obtain Wasserstein distance guarantees for any distribution of bounded support or sufficiently decaying tails, as well as TV guarantees for distributions with further smoothness assumptions.

==> packages-neurips.tex <==
%\usepackage{fullpage}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{bbm}
\usepackage{cancel}
\usepackage{hyperref}
\usepackage{thm-restate}
\usepackage{xypic}
%https://www.jmilne.org/not/Mxymatrix.pdf

\usepackage{algorithm}
\usepackage{algorithmicx,algpseudocode}


\usepackage{color}

\usepackage[backend=biber,style=alphabetic,maxbibnames=99]{biblatex}

==> predictor.tex <==
\section{Analysis for SGM based on reverse SDE's}
\label{s:pc-proof}

In this section, we analyze score-based generative models based on reverse SDE's. 
In Section~\ref{ss:p-1step}, we prove %the inequality for one-step error 
convergence of the predictor algorithm under $L^\iy$-accurate score estimate (Theorem~\ref{t:p-iy-simple}, restated as~\ref{t:p-iy}) using lemmas proved in Section~\ref{ss:diff-ineq},~\ref{ss:com}, \ref{ss:pert}, and \ref{ss:aux}.
In Section~\ref{ss:p-pf}, we prove convergence of the predictor algorithm under $L^2$-accurate score estimate
(Theorem~\ref{t:p}, restated as~\ref{t:p-precise}). In Section~\ref{ss:pc-pf}, we prove convergence of the predictor-corrector algorithm (Theorem~\ref{t:pc}).  

%\hlnote{Moved exposition to Section~\ref{s:pc}}
% Let $\Tilde{x}_t$ satisfies the (exact) forward SDE:
% \begin{equation}\label{general_forward_sde}
%     d\Tilde{x}_t 
%     = f(\Tilde{x}_t, t)dt + g(t)dw_t,\ t\in[0, T],
% \end{equation}
% where $w_t$ is a standard Brownian Motion and $\Tilde{x}_0\sim\Tilde{p}_0 = p_{data}$. Let $\Tilde{p}_t$ denote the distribution of $\Tilde{x}_t$, then $\Tilde{x}_t$ also satisfies the reverse-time SDE:
% \begin{equation}\label{general_reverse_sde}
%     d\Tilde{x}_t = [f(\Tilde{x}_t,t) - g(t)^2\nb\ln \Tilde{p}_t(\Tilde{x}_t)]dt + g(t)d\Tilde{w}_t,\ t\in[0, T],
% \end{equation}
% where $\Tilde{w}_t$ is a backward Brownian Motion. By carefully choosing $f$ and $g$, we can expect that $\Tilde{p}_T$ is approximately equal to some prior distribution (e.g. a centered Gaussian) which we can accurately sample from. Then we hope that starting with some $\Tilde{y}_T\sim \Tilde{q}_T\approx \Tilde{p}_T$ and running the reverse-time process, we will get a good sample $\Tilde{y}_0\sim\Tilde{q}_0\approx p_{data}$.


\subsection{Discretization and Score Estimation}\label{setting:C}
With a change of variable in~\eqref{general_reverse_sde}, we define the sampling process $x_t$ on $[0,T]$ by
\begin{align*}
    dx_t = [-f(x_t, T-t) + g(T-t)^2\nb\ln \Tilde{p}_{T-t}(x_t)]\,dt + g(T-t)\,dw_t,\ \ x_0\sim\Tilde{p}_T.
\end{align*}
Denoting the distribution of $x_t$ by $p_t$ and running the process from $0$ to $T$, we will exactly obtain  $p_T=\Tilde{p}_0$, which is the data distribution. In practice, we need to discretize this process and replace the score function $\nb\ln\Tilde{p}_{T-t}$ with the estimated score $\score$. With a general Euler-Maruyama method, we would obtain $\{z_k\}_{k=0}^N$ defined by
\begin{equation}\label{reverse_time_estimate_score}
   %\Tilde{z}_k = \Tilde{z}_{k+1} -
%    [f(\Tilde{z}_{k+1}, T-kh) - g(T-kh)^2\score (\Tilde{z}_{k+1}, T-kh)]h + \sqrt{h}g(T-kh)\eta_{k+1},
z_{(k+1)h} = z_{kh} -
    h\cdot [f(z_{kh}, T-kh) - g(T-kh)^2\score (z_{kh}, T-kh)] + \sqrt{h}\cdot g(T-kh)\eta_{k+1},
\end{equation}
where $h = T/N$ is the step size and $\eta_k$ is a sequence of independent Gaussian random vectors. As we run~\eqref{reverse_time_estimate_score} from $0$ to $N$ with $h$ small enough, we should expect that the distribution of $z_T$ is close to that of $x_T$. However, in both SMLD or DDPM models, for fixed $z_k$, the integration 
\begin{align*}
    \int_{kh}^{(k+1)h}f(z_{kh}, T-t)\,dt\ \ \text{and}\ \   \score(z_{kh}, T-kh)\cdot\int_{kh}^{(k+1)h}g(T-t)^2\,dt
\end{align*}
can be exactly computed, as can the diffusion term. Therefore, we can consider the following process $z_t$ as an ``interpolation'' of~\eqref{reverse_time_estimate_score}:
\begin{align}
    dz_t = [-f(z_{kh}, T-t) + g(T-t)^2 \score(z_{kh}, T-kh)]\,dt + g(T-t)\,dw_t,\ \ t\in[kh, (k+1)h].\label{z_t}
\end{align}
Note that by running this process instead, we can reduce the discretization error. Now if we denote the distribution of $z_t$ by $q_t$, with $q_0\approx p_0$, we can expect that $q_T$ is close to $p_T$. Here the estimated score $\score$ satisfies for all $x$
\begin{equation}
\label{e:Mkh}
    \ve{\score(x, T-kh)-\nb\ln \Tilde{p}_{T-kh}(x)} \leq \Mkh, \quad k=0,1,\ldots,N.
\end{equation}
Observe that in either SMLD or DDPM, the function $g(t)^2$ is Lipschitz on $[0,T]$. So in the following sections, we will assume that $g(t)^2$ is $L_g$-Lipschitz on $[0,T]$.


\subsection{Predictor}
\label{ss:p-1step}
In this section, we present the main result (Theorem~\ref{t:p-iy}) on the one-step error of the predictor in $\chi^2$-divergence, which can be obtained by directly applying the Gronwall's inequality to the differential inequality derived in Lemma~\ref{d_chi2}. Note that Theorem~\ref{t:p-iy} is a more precise version of Theorem~\ref{t:p-iy-simple}; see the remark following the theorem.

\begin{thm}\label{t:p-iy}
With the setting in Section~\ref{setting:C}, assume $g$ is non-decreasing and let
\begin{align*}
    0 < h \leq \min_{kh\le t\le (k+1)h}
    ??
\end{align*}
where $C_t$ is the log-Sobolev constant of $p_t$, bounded in Lemma~\ref{l:lsi-noise}. Suppose that $\nb \ln p_t$ is $L$-Lipschitz for all $t\in [kh,(k+1)h]$, $s(\cdot, kh)$ is $\sms$-Lipschitz, $L,\sms\ge 1$, and $\Mkh$ is such that~\eqref{e:Mkh} holds.
%the Lipschitz constant of both true and estimated score $L, L_s\geq 1$, we have
Then 
\begin{align*}
    \chi^2(q_{(k+1)h}||p_{(k+1)h}) \leq \ba{\chi^2(q_{kh}||p_{kh}) + ??}
    %\int_{kh}^{(k+1)h}C_{t,kh}\,dt}e^{\int_{kh}^{(k+1)h}(-\fc{1}{8C_t} + 8\Mkh^2)g(T-t)^2\,dt}
\end{align*}
\end{thm}

\fixme{[Rewrite rest of subsection.]}

\subsection{Differential Inequality}
\label{ss:diff-ineq}
Now we prove a differential inequality involving $\chi^2(q_t||p_t)$. As in \cite{chewi2021analysis}, the key difficulty is to bound the discretization error. We decompose it into two error terms and bound them in Lemma~\ref{l:error_A} and Lemma~\ref{l:error_B} separately.

In the following, we will let
\begin{align}
\label{e:Gkht}
    G_{kh,t}:&= \int_{kh}^t g(T-s)^2\,ds.
\end{align}

\begin{lem}\label{d_chi2}
Let $(q_t)_{0\leq t\leq T}$ denote the law of the interpolation~\eqref{z_t}. With the setting in Lemma~\ref{t:p-iy}, we have for $t\in[kh, (k+1)h]$,
\begin{align*}
    \fc{d}{dt}\chi^2(q_t||p_t)
    & \leq g(T-t)^2\ba{\pa{-\fc{1}{8C_t} + 8\Mkh^2}\chi^2(q_t||p_t) + \ba{8\Mkh^2 + \Etkh \cdot(t-kh)g(T-kh)^2}},
\end{align*}
where $C_t$ is the LSI constant of $p_t$, $\Mkh$ is the $L^\infty$-score estimation error at time $kh$ and $\Etkh $ is defined in~\eqref{constant:E_t_kh}.
\end{lem}
\begin{proof}
By Lemma~\ref{l:d-chi2} with
\begin{align*}
    \wh f(z_{kh},t) &\leftarrow -f(z_{kh}, T-t) + g(T-t)^2 s(z_{kh},T-kh)\\
    f(z,t) &\leftarrow -f(z,T-t) + g(T-t)^2 \nb \ln \wt p_{T-t}(z),
\end{align*}
we have
\begin{align*}
    \ddd t\chi^2(q_t||p_t)
    &= -g(T-t)^2 \sE_{p_t}\pf{q_t}{p_t} + 
    2\E\Big[\Big\langle 
    \pa{-f(z_{kh}, T-t) + g(T-t)^2 s(z_{kh}, T-kh)} \\
    &\quad - 
    \pa{-f(z,T-t) + g(T-t)^2 \nb \ln \wt p_{T-t}(z)}, \nb \fc{q_t}{p_t}\Big\rangle\Big]\\
    & = -g(T-t)^2\sE_{p_t}\pf{q_t}{p_t} + 2\E\ba{\an{f(z_t, T-t) - f(z_{kh}, T-t) ,\nb\fc{q_t(z_t)}{p_t(z_t)}}}\\
    &\ \ \ + 2g(T-t)^2\E\ba{\an{\score(z_{kh}, T-kh) -  \nb\ln\Tilde{p}_{T-t}(z_t), \nb\fc{q_t(z_t)}{p_t(z_t)}}}\\
    & =: -g(T-t)^2\sE_{p_t}\pf{q_t}{p_t} + A + B.
\end{align*}
By Lemma~\ref{l:error_A},
\begin{align*}
    A & \leq
        g(T-t)^2 \ba{2(\chi^2(q_t||p_t)+1) 
    \E\ba{\ve{z_t-z_{kh}}^2\psi_t(z_t)} + \rc{8} \sE_{p_t}\pf{q_t}{p_t}},
\end{align*}
while by Lemma~\ref{l:error_B},
\begin{align*}
    B 
    &\le
    g(T-t)^2 \Bigg\{
    8(\chiqpo)\ba{
    \sms^2 
    \E\ba{\ve{z_t-z_{kh}}^2\psi_t(z_t)} + \Mkh^2 + 
    \E\ba{\ve{\nb \ln p_{kh}(z_t) - \nb \ln p_t(z_t)}^2\psi_t(z_t)}} \\
    &\quad + \fc 38\FIqp
    \Bigg\}.
\end{align*}
Combining these inequalities gives
\begin{align*}
    \ddd t\chi^2(q_t||p_t)&\le 
    g(T-t)^2\Bigg\{
    -\rc 2 \FIqp + 2(\chiqpo)\Big[4\Mkh^2 + (4\sms^2+1) \Edz\\
    &\quad + 4\Edlnp
    \Big] 
    \Bigg\}\\
    &\le \cdots \\
    & \le 
    g(T-t)^2 \Bigg\{
    -\rc 2 \FIqp + 2(\chiqpo) \Bigg[
    8\Mkh^2 + (4\sms^2+1)\\
    &\quad \cdot 
    \pa{
    9\Gkht^2 \pa{\fc{2\FIqp}{\chiqpo} + dL + \rc 2 C_t \KLqp + \rc 4(M_t+C_t)} + 9\Gkht(4\KLqp + d + 8\ln 2)
    }
    \Bigg]
    \Bigg\}
\end{align*}
\fixme{[Rest of proof.]}
\end{proof}

\fixme{[Rest of section]}





 



